Detecting Abrupt Changes in Point Processes: Fundamental Limits and Applications

We consider the problem of detecting abrupt changes (i.e., large jump discontinuities) in the rate function of a point process. The rate function is assumed to be fully unknown, non-stationary, and may itself be a random process that depends on the history of event times. We show that abrupt changes can be accurately identified from observations of the point process, provided the changes are sharper than the "smoothness'' of the rate function before the abrupt change. This condition is also shown to be necessary from an information-theoretic point of view. We then apply our theory to several special cases of interest, including the detection of significant changes in piecewise smooth rate functions and detecting super-spreading events in epidemic models on graphs. Finally, we confirm the effectiveness of our methods through a detailed empirical analysis of both synthetic and real datasets.

==> cmds.tex <==
% COMMANDS AND HOTKEYS 
%\mathbb commands.
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\J}{\mathbb{J}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\usepackage{bbm}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\0}{\mathbbm{0}}

%\mathcal commands.
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Cs}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\ps}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\hbt}{\frac{\hbar}{2}}

%text shortcuts.
\newcommand{\dne}{\text{ DNE}}
\newcommand{\und}{\text{ undefined}}
\newcommand{\ad}{\text{ and }}
\newcommand{\fs}{\text{ for some }}
\newcommand{\we}{\text{ where }}
\newcommand{\wee}{\text{ where:}}
\newcommand{\st}{\text{ such that }}
\newcommand{\stt}{\text{ such that:}}
\newcommand{\wh}{\text{ we have }}
\newcommand{\wht}{\text{ we have that }}
\newcommand{\wi}{\text{ with }}
\newcommand{\el}{Euler-Lagrange Equation }
\newcommand{\eln}{Euler-Lagrange Equation}
\newcommand{\els}{Euler-Lagrange Equations }
\newcommand{\elsn}{Euler-Lagrange Equations}
\newcommand{\he}{Hamilton Equation }
\newcommand{\hen}{Hamilton Equation}
\newcommand{\hes}{Hamilton Equations }
\newcommand{\hesn}{Hamilton Equations}
\newcommand{\hje}{Hamilton-Jacobi Equation }
\newcommand{\hjen}{Hamilton-Jacobi Equation}
\newcommand{\sa}{$\sigma$-algebra }
\newcommand{\san}{$\sigma$-algebra}

%math single character shortcuts.
\newcommand{\fa}{\forall}
\newcommand{\eq}{\exists}
\newcommand{\imp}{\implies}
\newcommand{\dnimp}{\centernot\implies}
\newcommand{\cd}{\cdot}
\newcommand{\ceq}{\coloneqq} % :=
\newcommand{\sbs}{\subseteq}
\newcommand{\sps}{\supseteq}
\newcommand{\nsbs}{\not\subseteq}
\newcommand{\nsps}{\not\supseteq}
\newcommand{\nin}{\notin}
\newcommand{\sqsbs}{\sqsubseteq} % square subseteq

%math shortcut commands.
\newcommand{\Bp}{\B^\ast}
\newcommand{\f}{f^{-1}}
\newcommand{\e}{\varepsilon}
\newcommand{\de}{\delta}
\newcommand{\es}{\varnothing}
% \newcommand{\lp}{\ell^p}
\newcommand{\sm}{\setminus}
\newcommand{\p}{\partial}
\newcommand{\pr}{\, '}
% \newcommand{\indep}{\ensuremath{\! \! \perp \! \! \! \perp \!}}
\newcommand{\vf}{\vec{F}}
\newcommand{\vtau}{\vec{\tau}}
\newcommand{\vnab}{\vec{\nabla}} %vector gradient
\newcommand{\dotp}{\dot{\mathcal{P}}}
\newcommand{\dotq}{\dot{\mathcal{Q}}}
% \newcommand{\norm}{\| \circ \|}
\newcommand{\Co}{ \Cs \left( 0,1 \right) }
\newcommand{\Ca}{ \Cs \left( a,b \right) }
\newcommand{\FF}{ \{ F_\alpha \}_{\alpha \in I}}
\newcommand{\GG}{ \{ G_\alpha \}_{\alpha \in I}}
\newcommand{\HH}{ \{ H_\alpha \}_{\alpha \in I}}
\newcommand{\KK}{ \{ K_\alpha \}_{\alpha \in I}}
\newcommand{\Ro}{ \mathcal{R} \left( \left[ 0,1 \right] \right) }
\newcommand{\Ra}{ \mathcal{R} \left( \left[ a,b \right] \right) }
\newcommand{\UU}{ \{ U_\alpha \}_{\alpha \in I}}
\newcommand{\Vp}{\V^\ast}
\newcommand{\QC}{\R \sm \Q}
\newcommand{\Sigmast}{\Sigma^\ast}
\newcommand{\deast}{\de^\ast}
\newcommand{\De}{\Delta}
\newcommand{\Deast}{\De^{\hspace{-0.15 em}\ast}}
\newcommand{\Fhat}{\hat{F}}

% paired delimiters: 
\DeclarePairedDelimiter\absd{\lvert}{\rvert} % absolute val
\DeclarePairedDelimiter\normd{\lVert}{\rVert} % norm
\newcommand{\expectauto}[1]{\E\left[#1\right]} % expectation: auto adjusting
\newcommand{\cov}[1]{\operatorname{Cov}\left[#1\right]}
\newcommand{\corr}[1]{\operatorname{Corr}\left[#1\right]}

% automatic \left\right brackets 
\newcommand{\bpar}[1]{\left(#1\right)}
\newcommand{\bbr}[1]{\left[#1\right]}
\newcommand{\bcurly}[1]{\left\{#1\right\}}

% sums 
\newcommand{\sumlimin}{\sum_{i=1}^n}
\newcommand{\sumlimkn}{\sum_{k=1}^n}
\newcommand{\sumlimizn}{\sum_{i=0}^n}
\newcommand{\sumlimkzn}{\sum_{k=0}^n}
\newcommand{\sumlimyzinf}{\sum_{y=0}^\infty}
\newcommand{\sumlimyoinf}{\sum_{y=1}^\infty}
\newcommand{\sumlimiinf}{\sum_{i=-\infty}^\infty}
\newcommand{\intinfinf}{\int_{-\infty}^\infty }
\newcommand{\sumlimiN}{\sum_{i=1}^N}

%command shortcuts.
\newcommand{\ds}{\displaystyle}
\newcommand{\no}{\noindent}
\newcommand{\vs}{\vspace*}
\newcommand{\hs}{\hspace}
\newcommand{\bs}{\baselineskip}

% math operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\;max}

% probability things
% P(A | B) (given)
\newcommand\given[1][]{\:#1\vert\:}
\newcommand{\Bin}{\mathrm{Bin}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\ind}[1]{\1_{[#1]}} % indicator 
\newcommand{\bigind}[1]{\1_{\left[#1\right]}}  % big indicator
\newcommand{\disteq}{\stackrel{\L}{=}} % distributional equals

% hats and tildes 
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\itilde}{\Tilde{\imath}}


